Poisson equation in domains with concentrated holes

We consider solutions $u^\varepsilon$ of Poisson problems with the Dirichlet condition on domains $\Omega_\varepsilon$ with holes concentrated at subsets of a domain $\Omega$ non-periodically. We show $u^\varepsilon$ converges to a solution of a Poisson problem with a simple function potential. This is a generalized result of a sample model given by Cioranescu and Murat (1997). They showed a result for case that holes are distributed at $\Omega$ periodically.

==> resp.tex <==
\title{Response of the author to referees of SUTJM22-12}
\author[H. Ishida]{Hiroto Ishida}
\maketitle
Dear Editors and Referees

Thank you very much for your suggestions.

I changed title of the manuscript and applied your comments to the new manuscript  as much as I can.
However, some comments are not applied for some reasons.
I list these parts with reasons.

\paragraph{7. p.5 l.-12: unusual $\to$ nontrivial}
I don't want fix it since "unusual" is quote from $[1]$.
I fixed the sentence contain "unusual" to avoid misunderstanding.
If the fixed sentence doesn't make sense, I remove the sentence.
\paragraph{9. p.8 ll8-10:Insert commas and a period}
I couldn't understand reason. Maybe, I lack of understanding about usage of commas.
\paragraph{9. p.8 proof of Lemma 8:on $\Omega\to$ in $\Omega$}
I couldn't understand reason. I used the words "on $\Omega$" at everywhere of the manuscript. Should I also fix them to "in $\Omega$"? 
\paragraph{9. (3.2)}
$\pd_r q_0^\ep$ is function on $[0,C\ep].$ (It is not directional derivative of $q^\ep.$)

I'm sorry if I misunderstanding your suggestions.

Sincerely yours,

Hiroto Ishida
